The Word2vec Graph Model for Author Attribution and Genre Detection in Literary Analysis

Analyzing the writing styles of authors and articles is a key to supporting various literary analyses such as author attribution and genre detection. Over the years, rich sets of features that include stylometry, bag-of-words, n-grams have been widely used to perform such analysis. However, the effectiveness of these features largely depends on the linguistic aspects of a particular language and datasets specific characteristics. Consequently, techniques based on these feature sets cannot give desired results across domains. In this paper, we propose a novel Word2vec graph based modeling of a document that can rightly capture both context and style of the document. By using these Word2vec graph based features, we perform classification to perform author attribution and genre detection tasks. Our detailed experimental study with a comprehensive set of literary writings shows the effectiveness of this method over traditional feature based approaches. Our code and data are publicly available at https://cutt.ly/svLjSgk

==> backup_table.tex <==
\begin{table*}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Feature set}}} & \multicolumn{2}{c|}{\textbf{Author Attribution}}                      & \multicolumn{2}{c|}{\textbf{Genre Detection}}                         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                      & \multicolumn{1}{c|}{\textbf{SVM}} & \multicolumn{1}{c|}{\textbf{kNN}} & \multicolumn{1}{c|}{\textbf{SVM}} & \multicolumn{1}{c|}{\textbf{kNN}} \\ \hline
w2v graph                                                   & 75.28                             & 31.11                             & 87.14                             & 48.89                             \\ \hline
w2v graph (s)                                               & 65.63                             & 30.95                             & 79.14                             & 54.32                             \\ \hline
w2v graph+ graph words                                      & 81.40                             & 43.88                             & \textbf{92.30}                    & 56.62                             \\ \hline
w2v graph (s)+ graph words                                  & 83.77                             & 43.48                             & 81.45                             & 48.55                             \\ \hline
TF-IDF                                                      & 43.62                             & 57.94                             & 85.43                             & 50.43                             \\ \hline
TF-IDF (s)                                                  & 42.38                             & 47.70                             & 87.30                             & 39.04                             \\ \hline
TF-IDF (top 100 words)                                      & 36.34                             & 36.91                             & 88.83                             & 55.97                             \\ \hline
Stylometry                                                  & 52.65                             & 29.22                             & 87.40                             & 85.99                             \\ \hline
Multilingual BERT                                           & \textbf{85.98}                    & 41.47                             & 62.22                             & 44.74                             \\ \hline
AVG of w2v vectors                                          & 75.49                             & 41.47                             & 78.40                             & 47.65                             \\ \hline
AVG of w2v vectors (s)                                      & 78.41                             & 41.47                             & 89.14                             & 47.65                             \\ \hline
w2v graph words only                                        &                                   &                                   & 46.33                             & 52.01                             \\ \hline
\end{tabular}
\end{table*}
